Convex programming in optimal control and information theory

The main theme of this thesis is the development of computational methods for classes of infinite-dimensional optimization problems arising in optimal control and information theory. The first part of the thesis is concerned with the optimal control of discrete-time continuous space Markov decision processes (MDP). The second part is centred around two fundamental problems in information theory that can be expressed as optimization problems: the channel capacity problem as well as the entropy maximization subject to moment constraints.

==> RL.tex <==
% ensures that the main file is compiled
% !TEX root = ../Thesis.tex 


%%% File encoding is ISO-8859-1 (also known as Latin-1)
%%% You can use special characters just like ä,ü and ñ

% Chapter without numbering but with appearance in the Table of Contents
% \addchap is a command from KOMA-Script




\chapter{Reinforcement learning setting}

blabla


